Interpolation and Amalgamation for Arrays with MaxDiff (Extended Version)

In this paper, the theory of McCarthy's extensional arrays enriched with a maxdiff operation (this operation returns the biggest index where two given arrays differ) is proposed. It is known from the literature that a diff operation is required for the theory of arrays in order to enjoy the Craig interpolation property at the quantifier-free level. However, the diff operation introduced in the literature is merely instrumental to this purpose and has only a purely formal meaning (it is obtained from the Skolemization of the extensionality axiom). Our maxdiff operation significantly increases the level of expressivity; however, obtaining interpolation results for the resulting theory becomes a surprisingly hard task. We obtain such results via a thorough semantic analysis of the models of the theory and of their amalgamation properties. The results are modular with respect to the index theory and it is shown how to convert them into concrete interpolation algorithms via a hierarchical approach.

==> macros-common.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Time-stamp: "2018-05-04 19:54:00 calvanese"
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%% General Math

\newcommand{\A}{\ensuremath{\mathcal{A}}}
\newcommand{\B}{\ensuremath{\mathcal{B}}}
\newcommand{\C}{\ensuremath{\mathcal{C}}}
\newcommand{\D}{\ensuremath{\mathcal{D}}}
\newcommand{\E}{\ensuremath{\mathcal{E}}}
\newcommand{\F}{\ensuremath{\mathcal{F}}}
\newcommand{\G}{\ensuremath{\mathcal{G}}}
\renewcommand{\H}{\ensuremath{\mathcal{H}}}
\newcommand{\I}{\ensuremath{\mathcal{I}}}
\newcommand{\J}{\ensuremath{\mathcal{J}}}
\newcommand{\K}{\ensuremath{\mathcal{K}}}
\renewcommand{\L}{\ensuremath{\mathcal{L}}}
\newcommand{\M}{\ensuremath{\mathcal{M}}}
\newcommand{\N}{\ensuremath{\mathcal{N}}}
\renewcommand{\O}{\ensuremath{\mathcal{O}}}
\renewcommand{\P}{\ensuremath{\mathcal{P}}}
\newcommand{\Q}{\ensuremath{\mathcal{Q}}}
\newcommand{\R}{\ensuremath{\mathcal{R}}}
\renewcommand{\S}{\ensuremath{\mathcal{S}}}
%\newcommand{\T}{\ensuremath{\mathcal{T}}}
\newcommand{\U}{\ensuremath{\mathcal{U}}}
\newcommand{\V}{\ensuremath{\mathcal{V}}}
\newcommand{\W}{\ensuremath{\mathcal{W}}}
\newcommand{\X}{\ensuremath{\mathcal{X}}}
\newcommand{\Y}{\ensuremath{\mathcal{Y}}}
\newcommand{\Z}{\ensuremath{\mathcal{Z}}}

%%%%%%%%%%%%%%%%%%%%%%%%%% Abbreviations

%%\newcommand{\eset}{\emptyset}
%%\newcommand{\col}{\colon}
\newcommand{\ol}[1]{\overline{#1}}                % overline
%\newcommand{\ul}[1]{\underline{#1}}               % underline
%%\newcommand{\uls}[1]{\underline{\raisebox{0pt}[0pt][0.45ex]{}#1}}
%% ul with space between text and line

\newcommand{\ra}{\rightarrow}
\newcommand{\Ra}{\Rightarrow}
%\newcommand{\la}{\leftarrow}
\newcommand{\La}{\Leftarrow}
%\newcommand{\lra}{\leftrightarrow}
\newcommand{\Lra}{\Leftrightarrow}
\newcommand{\lora}{\longrightarrow}
\newcommand{\Lora}{\Longrightarrow}
\newcommand{\lola}{\longleftarrow}
\newcommand{\Lola}{\Longleftarrow}
\newcommand{\lolra}{\longleftrightarrow}
\newcommand{\Lolra}{\Longleftrightarrow}
%\newcommand{\ua}{\uparrow}
\newcommand{\Ua}{\Uparrow}
\newcommand{\da}{\downarrow}
\newcommand{\Da}{\Downarrow}
\newcommand{\uda}{\updownarrow}
\newcommand{\Uda}{\Updownarrow}

%%%%%%%%%%%%%%%%%%%%%%%%%% Relations

%%\newcommand{\incl}{\subseteq}
%%\newcommand{\imp}{\rightarrow}
\newcommand{\per}{\mbox{\bf .}}                  % period

%%%%%%%%%%%%%%%%%%%%%%%%%% Delimiters

%%\newcommand{\quotes}[1]{{\lq\lq #1\rq\rq}}
\newcommand{\set}[1]{\{#1\}}                      % set
\newcommand{\Set}[1]{\left\{#1\right\}}
\newcommand{\bigset}[1]{\Bigl\{#1\Bigr\}}
\newcommand{\bigmid}{\Big|}
\newcommand{\size}[1]{|{#1}|}                     % cardinality of a set
%%\newcommand{\Card}[1]{\left| #1\right|}
%\newcommand{\card}[1]{\sharp #1}
%\newcommand{\tup}[1]{\langle #1\rangle}            % tuple
%\newcommand{\Tup}[1]{\left\langle #1\right\rangle}

\newcommand{\setone}[2][1]{\set{#1\cld #2}}

%%%%%%%%%%%%%%%%%%%%%%%%%% STYLING AND SPACING
\newcolumntype{C}{>{\centering\arraybackslash}X}

\makeatletter
\g@addto@macro\normalsize{%
\setlength{\abovecaptionskip}{-2pt}
\setlength\abovedisplayskip{3pt}
\setlength\belowdisplayskip{3pt}
\setlength\abovedisplayshortskip{3pt}
\setlength\belowdisplayshortskip{3pt}
}
\makeatother

\newcounter{dummy} 
\newcounter{dummy1} 
\newcounter{dummy2}
\newcounter{dummy3} 
\newcounter{dummy4}
\newcounter{dummy5} 
\newcounter{dummy6}
%\numberwithin{dummy}{section}

\usepackage[thmmarks,amsmath]{ntheorem}
\theorempreskip{1pt}
\theorempostskip{1pt}

%\theoremstyle{plain}
%\theorembodyfont{\normalfont}
%\theoremseparator{.}
%\let\definition\relax
%\theoremsymbol{\ensuremath{\square}}
%\newtheorem{definition}{Definition}


\let\proposition\relax
\let\theorem\relax
\let\lemma\relax
\let\definition\relax
\theoremseparator{.}
\theorembodyfont{\itshape}
\theoremsymbol{$\triangleleft$}
\newtheorem{theorem}[dummy]{Theorem}
\newtheorem{lemma}[dummy1]{Lemma}
\newtheorem{definition}[dummy2]{Definition}
\newtheorem{proposition}[dummy3]{Proposition}

\let\example\relax
\let\remark\relax
\theorembodyfont{\normalfont}
\newtheorem{example}[dummy4]{Example}
\newtheorem{remark}[dummy5]{Remark}


\theoremstyle{nonumberplain}
\theoremheaderfont{\itshape}
\theorembodyfont{\normalfont}
\let\proof\relax
\theoremseparator{.}
\theoremsymbol{\ensuremath{\dashv}}
\newtheorem{proof}[dummy6]{Proof}


\qedsymbol{\ensuremath{\dashv}}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% save-place: t
%%% End:


==> macros.tex <==
\newcommand{\st}{\; \vert \;}
\newcommand{\idx}[2][i]{\ensuremath {#1 \in \{1,\ldots,\mbox{$#2$}\}}}

\newcommand{\ua}{\ensuremath{\underline a}}
\newcommand{\ub}{\ensuremath{\underline b}}
\newcommand{\uc}{\ensuremath{\underline c}}
\newcommand{\ud}{\ensuremath{\underline d}}
\newcommand{\ue}{\ensuremath{\underline e}}
\newcommand{\ui}{\ensuremath{\underline i}}
\newcommand{\uu}{\ensuremath{\underline u}}
\newcommand{\ut}{\ensuremath{\underline t}}
\newcommand{\uv}{\ensuremath{\underline v}}
\newcommand{\ux}{\ensuremath{\underline x}}
\newcommand{\uy}{\ensuremath{\underline y}}
\newcommand{\uz}{\ensuremath{\underline z}}
\newcommand{\uF}{\ensuremath{\underline F}}
\newcommand{\uG}{\ensuremath{\underline G}}
\newcommand{\uS}{\ensuremath{\underline S}}

\newcommand{\PSPACE}{\textsc{Pspace}\xspace}

%\renewcommand{\qedsymbol}{$\dashv$}
\newcommand{\cA}{\ensuremath \mathcal A}
\newcommand{\cC}{\ensuremath \mathcal C}
\newcommand{\cB}{\ensuremath \mathcal B}
\newcommand{\cM}{\ensuremath \mathcal M}
\newcommand{\cN}{\ensuremath \mathcal N}
\newcommand{\cS}{\ensuremath \mathcal S}
\newcommand{\cT}{\ensuremath \mathcal T}
\newcommand{\cI}{\ensuremath \mathcal I}
\newcommand{\lra}{\longrightarrow}

\newcommand{\lnext}{\ensuremath X}
\newcommand{\lbox}{\ensuremath \Box}
\newcommand{\ldiamond}{\ensuremath \Diamond}
\newcommand{\luntil}{\ensuremath U}
\newcommand{\lrelease}{\ensuremath R}

\newcommand{\ltl}{LTL}
\newcommand{\safe}{\texttt{SAFE}\xspace}
\newcommand{\unsafe}{\texttt{UNSAFE}\xspace}
\newcommand{\mcmt}{\textsc{mcmt}\xspace}


%\newcommand{\ltl}{\textit{LTLT}}
\newcommand{\ltlt}{\ltl(\ensuremath {\mathcal T})}
\newcommand{\dpllt}{\textit{DPLL}(\ensuremath {\mathcal T})}
\newcommand{\ltlfor}{\ltl($\Sigma^{\ua}$)}
\newcommand{\ltlforci}{\ltl($\Sigma^{\uc}$)}
\newcommand{\ltlforc}{\ltl($\Sigma^{\ua, \uc}$)}

\newcommand{\abstr}[1][\varphi]{\ensuremath {\lbrack\!\lbrack\, #1 \,\rbrack\!\rbrack}}
\renewcommand{\int}{\ensuremath {\mathcal I}}
\newcommand{\closure}{\ensuremath {cl}}
\newcommand{\pre}[1][T]{\ensuremath {Res_{#1}}}
\newcommand{\disjcup}{\ensuremath \oplus}
\newcommand{\bigdisjcup}{\ensuremath \bigoplus}
\newcommand{\sysset}{\ensuremath {\langle \Sigma, T, \Sigma_r, \ua, \uc \rangle}}
\newcommand{\sysspec}{\ensuremath {(\mathcal T, \delta, \iota)}}

\newcommand{\satproc}{\textit{``satisfiable''}}
\newcommand{\unsatproc}{\textit{``unsatisfiable''}}
\newcommand{\prename}{residue enumerator}
\newcommand{\pbename}{\prename}

\newcommand{\theory}{data-flow theory}
\newcommand{\theories}{data-flow theories}

\newcommand{\theoryCADE}{\ltl-theory}
\newcommand{\theoriesCADE}{\ltl-theories}

\renewcommand{\sp}{\ensuremath{\mathcal{SP}}}

\newcommand{\EUF}{\ensuremath{\mathcal{EUF}}}

\newcommand{\limplies}{\ensuremath{\Rightarrow}}
\renewcommand{\lnot}{\ensuremath{\sim}}
\renewcommand{\iff}{\ensuremath{\Leftrightarrow}}


\newcommand{\BA}{\ensuremath{BA}}

\newcommand{\domain}[1]{\mathit{dom}(#1)}
\newcommand{\image}[1]{\mathit{imm}(#1)}


%%%%%% MACRO SUI NOMI %%%%%%%

\newcommand{\aas}{AAS\xspace}
\newcommand{\AAS}{Abstract Artifact System\xspace}

\newcommand{\sas}{SAS\xspace}
\newcommand{\SAS}{Simple Artifact System\xspace}

\newcommand{\ras}{RAS\xspace}
\newcommand{\RAS}{Relational Artifact System\xspace}

\newcommand{\mem}{\W}


\newcommand{\type}[1]{\ensuremath{\mathsf{#1}}\xspace}
\newcommand{\funct}[1]{\ensuremath{\mathit{#1}}\xspace}
\newcommand{\relname}[1]{\ensuremath{\mathit{#1}}\xspace}
\newcommand{\attrname}[1]{\funct{#1}}
\newcommand{\constant}[1]{\texttt{#1}}

\newcommand{\rels}[1]{#1_{\mathit{rel}}}
\newcommand{\sorts}[1]{#1_{\mathit{srt}}}
\newcommand{\functs}[1]{#1_{\mathit{fun}}}
\newcommand{\vals}[1]{#1_{\mathit{val}}}
\newcommand{\ids}[1]{#1_{\mathit{ids}}}
\newcommand{\ext}[1]{#1_{\mathit{ext}}}

\newcommand{\nullv}{\texttt{undef}}

\newcommand{\lentry}[2]{\ensuremath{#1\,{:}\,#2}}
%%%%%%%%%%% TIKZ %%%%%%%%%%



\definecolor{deepblue}{HTML}{0C3B80}
\definecolor{deepgreen}{HTML}{2EA601}
%\definecolor{deepblue}{HTML}{232F3E}
%\definecolor{chaptercolor}{HTML}{232F3E}{0.8}
\definecolor{lightOrange}{HTML}{FFA03C}
\definecolor{darkOrange}{HTML}{F1800A}
\definecolor{lightBlue}{HTML}{0174CD}
\definecolor{greenF}{HTML}{2CBB5C}
\definecolor{cyan}{HTML}{86A6D5}


\tikzstyle{sortnode} = [
  rectangle,
  rounded corners=5pt,
  minimum width=18mm,
  minimum height=6mm,
  very thick,
]

\tikzstyle{functnode} = [
  rectangle,
  minimum width=1cm,
  minimum height=5mm,
]

\tikzstyle{idnode} = [
  sortnode,
  draw=deepblue,
  fill=cyan!50,
  text=deepblue,  
]

\tikzstyle{valnode} = [
  sortnode,
  densely dashed,
  draw=violet,
  fill=magenta!50,
  text=violet,
]

\tikzstyle{f} = [
  thick,
]

\tikzstyle{fd} = [
  f,
  -angle 90,
]

\tikzstyle{relation}=[rectangle split, rectangle split parts=#1, rectangle split part align=base, draw, anchor=center, align=center, text height=3mm, font=\bfseries, text centered]

%%%%%%% SMT %%%%%%%%%%
\newcommand{\smtlambda}[2]{
  \lambda #1.\left(#2\right)
}
\newcommand{\smtif}[4]{
  \begin{array}[#1]{@{}l@{}}
  \mathsf{if~}#2\mathsf{~then~}#3
  \\\mathsf{else~}#4
  \end{array}
}

\newcommand{\smtifinline}[3]{
  \mathsf{if~}#1\mathsf{~then~}#2\mathsf{~else~}#3
}

\newcommand{\typedvar}[2]{#1{:}#2}


%%%%%%% EXAMPLE %%%%%%%%%%

\newcommand{\artvar}[1]{\mathit{#1}}


\newcommand{\hrsig}{\Sigma_{\mathit{hr}}}
\newcommand{\hrras}{\S_{\mathit{hr}}}
\newcommand{\userid}{\type{UserId}}
\newcommand{\jobcatid}{\type{JobCatId}}
\newcommand{\empid}{\type{EmpId}}
\newcommand{\compinid}{\type{CompInId}}
\newcommand{\stringval}{\type{String}}


\newcommand{\username}{\funct{userName}}
\newcommand{\empname}{\funct{empName}}
\newcommand{\compemp}{\funct{who}}
\newcommand{\compjob}{\funct{what}}
\newcommand{\jobdescr}{\funct{jobCatDescr}}


\newcommand{\pstatev}{\artvar{pState}}
\newcommand{\uidv}{\artvar{uId}}





\newcommand{\jid}{\artvar{jId}}
\newcommand{\dval}{\artvar{pubDate}}
\newcommand{\ostate}{\artvar{pubState}}
\newcommand{\recstate}{\artvar{aState}}
\newcommand{\uid}{\artvar{uId}}
\newcommand{\eid}{\artvar{eid}}


\newcommand{\enab}{\constant{enabled}}
\newcommand{\publishing}{\constant{publishing}}
\newcommand{\published}{\constant{published}}
\newcommand{\joopen}{\constant{open}}
\newcommand{\joclosed}{\constant{closed}}
\newcommand{\joselected}{\constant{joSelected}}
\newcommand{\appreceived}{\constant{received}}
\newcommand{\win}{\constant{winner}}
\newcommand{\los}{\constant{loser}}
\newcommand{\final}{\constant{final}}
\newcommand{\notified}{\constant{notified}}


\newcommand{\joidx}{\type{joIndex}}
\newcommand{\jocat}{\funct{joCat}}
\newcommand{\jodate}{\funct{joPDate}}
\newcommand{\jostate}{\funct{joState}}



\newcommand{\appidx}{\type{appIndex}}
\newcommand{\appjob}{\funct{appJobCat}}
\newcommand{\appuser}{\funct{applicant}}
\newcommand{\appresp}{\funct{appResp}}
\newcommand{\appscore}{\funct{appScore}}
\newcommand{\appres}{\funct{appResult}}
\newcommand{\scoreval}{\type{Score}}



%%%% CHARACTERISTIC GRAPH %%%%

\tikzstyle{sortnode} = [
  rectangle,
  rounded corners=5pt,
  minimum width=18mm,
  minimum height=6mm,
  very thick,
]

\tikzstyle{functnode} = [
  rectangle,
  minimum width=1cm,
  minimum height=5mm,
]

\tikzstyle{idnode} = [
  sortnode,
  draw=deepblue,
  fill=cyan!50,
  text=deepblue,  
]

\tikzstyle{artnode} = [
  sortnode,
  draw=deepblue,
  fill=yellow!50,
  text=deepblue,  
]

\tikzstyle{valnode} = [
  sortnode,
  densely dashed,
  draw=violet,
  fill=magenta!50,
  text=violet,
]

\tikzstyle{f} = [
  thick,
]

\tikzstyle{fd} = [
  f,
  -angle 90,
]

\tikzstyle{relation}=[rectangle split, rectangle split parts=#1, rectangle split part align=base, draw, anchor=center, align=center, text height=3mm, font=\bfseries, text centered]


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

